CMB-S4 Science Case, Reference Design, and Project Plan

We present the science case, reference design, and project plan for the Stage-4 ground-based cosmic microwave background experiment CMB-S4.

==> Science/Dark_Energy_and_Dark_Matter.tex <==
\section{Dark Energy and Dark Matter}
%Proposed chapter name change: Dark Sector Constraints
\label{sec:DEDM}

\input Science/Dark_Matter.tex
\input Science/Dark_Energy.tex




==> Science/ScienceGoalsSummaryv2.tex <==
\section{Summary of Science Goals}

We have organized our diverse set of scientific goals into five themes: primordial gravitational waves, light relics, mass mapping, baryon mapping, and time domain exploration. The first two science themes have been primary drivers of the CMB-S4 concept since before Snowmass. The next three themes have emerged more recently as our understanding of the broader scientific opportunities has matured. We refer to them collectively as our Legacy Survey Themes. In this summary we articulate our primary goals in each of these themes, leaving further (and more detailed) explication of the full science case to the remainder of the chapter.

\subsection{Primordial Gravitational Waves and Density Perturbations}

{\bf Should this section be broader than PGW and also include something about PDP?}

We see a historic opportunity to open the gravitational wave window to the primordial universe. CMB-S4 will deliver a detection of primordial gravitational waves if the predictions of some of the leading models for the origin of the hot big bang are borne out. A detection would reveal a new scale of high energy physics near the GUT scale, provide the first evidence for the quantization of gravity, yield insight into the symmetries of nature and possibly even into deep properties of quantum gravity. A null result would force a dramatic shift in our understanding of basic early universe cosmology.

These leading models are models of cosmic inflation, a period of accelerated expansion preceding the hot big bang. Although we cannot yet claim with high confidence that the universe underwent cosmic inflation, the predictions of the simplest models of inflation have met with much empirical success. These predictions include small mean spatial curvature, a spectrum of density pertubrations that is nearly scale-invariant (but not completely scale invariant), adiabatic, and Gaussian, and acoustic peaks in the CMB angular power spectra. All of these predictions have been verified to high precision. 

The observed small departure from scale invariance of the density perturbations has quantitative implications for the detectability of primordial gravitational waves. All models that naturally explain the departure, and that have a scalar field effective potential with a super-Planckian mass scale (we need a better way to say this), generate tensor perturbations above the 95\% confidence upper limit that CMB-S4 can set. A special sub-class within this set of models is detectable by CMB-S4 at 5$\sigma$. 

Due to extreme amounts of expansion since the relevant length scales exited the horizon during the inflationary epoch, CMB observations probe physics at length scales up to $10^{10}$ times smaller than those probed in terrestrial colliders. Indeed, while the previous decade of work brought about the successful operation of the Large Hadron Collider and discovery of the Higgs, the lack of new physics signatures in colliders brings renewed importance to pursuing cosmological probes of high energy physics. The observational goal that will allow new phenomena to be tested through the CMB is clear: we must measure the polarization to high precision on angular scales from several minutes arc, to degrees.

By measuring at multiple frequencies to allow for the removal of galactic foreground contamination, and by measuring at small angular scales to allow for removal of gravitational lensing-generated polarization B modes, we will detect or tightly constrain the degree-scale B modes generated by gravitational waves, allowing us to detect or set an upper limit on the tensor-to-scalar ratio $r$. With an order of magnitude more detectors than precursor observations, and exquisite control of systematic errors, we will improve upon limits from precursor observations by more than a factor of 3, allowing us to either detect primordial gravitational waves or close out the super-Planckian window. 

What about primordial density perturbations and fNL? 


Should probably move an $n_s$ vs. $r$ figure into this subsection.

\subsection{Light Relics}

Cosmology unites the study of the fundamental laws of particle physics, the history of the universe, the origin of its structure, and its subsequent dynamics.  
The abundances of baryons, photons, neutrinos, and (possibly) dark matter were determined during the hot thermal phase that dominated the early universe. 
It is the abundances of these particles and the forces between them that determine the conditions of the universe that we see today. 

To date, cosmological observations have revealed to us a dark sector with at least two components: dark matter and dark energy. 

To date we can probe the creation of particles back to the first few seconds of the expansion, when neutrinos decoupled from the plasma. Although the cosmic neutrino background has not been directly detected, we have seen the influence of its energy density and free-streaming propagation on CMB temperature and polarization anisotropies at high significance, as well as on the abundances of light elements. 

With CMB-S4 we have the opportunity to probe the thermal history of the universe to much earier times: small fractions of a second, with plasma temperatures 

There is strong motivation to determine if there is more to this list of ingredients, in particular more light particles produced in thermal equilibrium. 
Many extensions of the Standard Model~(SM) predict new light particles, including axions, sterile neutrinos, and many solutions of the hierarchy problem (e.g.~supersymmetry)~\cite{Abazajian:2012ys, Essig:2013lka, Alexander:2016aln}. For large regions of unexplored parameter space these light particles are thermalized in the early universe. 

These types of light particles are ubiquitous in models of the late universe as well.  They may form the dark matter (e.g.~axions), be an essential ingredient of a more complicated dark sector as the force carrier between dark matter and the Standard Model (or itself), or provide a source of dark radiation for a dark thermal history.  Furthermore, they could explain discrepancies in the measurements of the Hubble constant~$H_0$, the amplitude of large-scale matter fluctuations~$\sigma_8$, and the properties of clustering on small scales.  

Remarkably, cosmology is providing an increasingly sharp view of these possibilities.  The cosmic neutrino background itself is a compelling example: while it has not been possible to see cosmic neutrinos in the lab, the influence of their energy density, and free-streaming evolution,  has been observed at high significance in the cosmic microwave background~(CMB) and primordial abundances of light elements. CMB obervations to date have provided us with a window back to a few seconds after the big bang (the era of neutrino decoupling). With CMB-S4  but also implies that any new light particles must be more weakly interacting than these neutrinos.

\subsection{Mapping mass in the universe}

Gravitational lensing of background sources by intervening gravitational potentials leads
to detectable distortions that can be used to reconstruct fluctuations in the
mass density. Using the CMB as a background source, virtually all of the the density 
fluctuations within the observable universe leave an imprint in the CMB.

The map resulting from CMB lensing reconstruction should be wide-area, highly sensitive,
and extremely well-calibrated.

On its own, this map can be used to measure the amplitude of large scale
structure at intermediate redshifts, with important applications to dark energy 
studies of neutrino masses. 

This map can be used to weigh samples of galaxies and galaxy clusters to as high a
redshift as such sources can be found. 

In conjunction with cosmic shear surveys (e.g., LSST) a map of the high-redshift
mass distribution can be constructed, while detailed comparison of lensing by
low-z structure of both the CMB and intermediate-z galaxies 
provides cross-checks on galaxy shear measurements and geometric tests.

\subsection{Mapping ionized gas in the universe}

Most of the baryons in the late universe are believed to be in a diffuse ionized plasma 
that is difficult to observe. This ionized plasma can leave imprints in the CMB
through Compton scattering, the so-called Sunyaev-Zeldovich effect. The two leading
effects are either a spectral distortion from hot electrons interacting with the
relatively cold CMB (tSZ), or a general redshift or blueshift of the scattered
photons due to coherent bulk flows along the line of sight (kSZ). 

With good frequency coverage, it is possible to measure the tSZ everywhere on the sky
and make a temperature-weighted map of the cosmic ionized gas fluctuations. The nature
of the scattering makes the measured distortion independent of redshift, providing
a means to detect large concentrations of hot electrons (galaxy clusters)
out to high redshift. This map can also be used to measure the average
thermal pressure profiles (in projection) around catalogs of 
galaxies and groups of galaxies.

The kSZ effect is on average very small along a given sightline, as there is an equal
number of motions toward us as away from us. To break this cancellation, 
information from other large scale structure surveys can be used. When including 
information from these other surveys (either spectroscopic or photometric galaxy
surveys can be used), it is possible to map the ionized gas that is associated
with the chosen galaxy sample. Applications of these maps are widely varied:
the measured ionized gas as a function of distance can be used to directly constrain
the impact of feedback from active galactic nuclei and supernovae on the 
intergalactic medium; the bulk flow amplitude as a function of separation can be
used to put constraints on theories of modified gravity; the large scale bulk flows
can be used as a unique measurement of large scale clustering on scales that are
difficult to reliably constrain using galaxy surveys.

Even without overlapping galaxy catalogs, the kSZ signal adds extra small-scale
power to the CMB power spectrum, and the structure is significantly non-Gaussian.
Some of this excess power and non-Gaussianity will be coming from the relatively
local universe where the galaxy catalogs overlap, but there should be a large
signal coming from the epoch of reionization. By directly probing the ionized
gas distribution, these measurements are completely complementary to the 
measurements of the neutral gas that can be obtained with redshifted Ly-$\alpha$
or redshifted 21-cm studies.

\subsection{The time-variable mm-wave sky}

There have been relatively few studies of the variable sky at mm-wavelengths. 
Known contributors to the time-varying sky are transient events, solar system
objects, and variable active galactic nuclei (especially blazars).


Pointed follow-up of gamma-ray bursts, core-collapse supernovae, tidal disuption events,
classical novae, and stellar flares have found that there are many transient events
detectable at these wavelengths.  A systematic survey of the mm-wave sky with a
cadence of a day or two over a large fraction of the sky would be an excellent
complement to other transient surveys, filling a gap between radio and optical
searches. The natural wide-area nature of the survey will make it straightforward
to search for gravitational wave sources that happen to be poorly localized.

Thermal emission from planets, 
dwarf planets, and asteroids have been measured at these wavelengths, and as these
sources move across the sky they should be easily differentiated from the 
relatively stationary extrasolar sky. Using the thermal emission rather than
reflected light has several complementary aspects: the fall-off with distance is less severe,
providing unique information on possible large objects in the distant reaches of
the solar system; the physical information available is very different, 
measuring long-wavelength emissivity rather than optical reflectivity; and with long
baselines for observation it will be possible to build up rotation curves for many 
objects, for detailed comparison with the optical versions.

Accreting black holes are known to be highly variable. A CMB survey can provide
a long baseline with high time sampling in both intensity and linear polarization.
This will provide an archive for multimessenger astronomy, in particular for
future blazars that are discovered to be sources of high-energy neutrinos.
With a large catalog of time-variable blazars, it will be possible to derive
detailed variability statistics over several years with nearly daily monitoring for 
both the detected objects and the sources that are observed to not be neutrino sources.





==> Science/legacy_catalogs/galaxy_variable.tex <==
\subsubsection{The Variable Galaxy:} %[Doug Johnstone]

Protostellar variability
offers a unique insight into the mass-accretion history of protostars.
There is a fundamental disconnect between steady-state star-formation models
and observed protostars -- we know that at least some protostars go through
explosive burst events during their evolution and that this may be important
for the overall mass assembly (e.g., \cite{Armitage2015}.
Circumstantial evidence suggests
that most, if not all, protostars go through these stages; however,
given the rarity of these large bursts, to catch one requires monitoring
a huge number of protostars (thousands) over many years.  CMB-S4 provides
that opportunity.

A survey with the James Clerk Maxwell Telescope \cite{Johnstone2018}
has found that about 10\% of protostars show low-level accretion variability,
over timescales of a year or so \cite{Mairs2017}.  This strongly suggests
that we are probing physical conditions in
the inner, planet-forming, disk.  In at least one case quasi-periodicity is
seen over many years, suggesting a link to long-lived structure (i.e.,
companions or planets) within the disk.
Additionally protostars are expected to be very active and a handful of
extremely powerful flares have been observed in the radio
\cite{Forbrich2017}.  Magnetic fields
are believed to play an important role in funneling material from the disk
onto the star (the last step for accretion).  Detailed measurements of the
properties of magnetic reconnection events are required to make significant
progress in our understanding of this complex phenomenon.  Follow-up
spectroscopic studies of flares discovered with CMB-S4 could unveil the
astrochemsitry of the time-varying signatures of volatile species and
UV and X-ray dissociation, as well as changes in the protoplanetary disk
snow-line through evaporation of ices.

These examples illustrate that there are important physical processes that
can be discerned through measurements of variability and transient phenomena
within the Milky Way.  At millimeter wavelengths, so far only one modest
survey (the JCMT Transient Survey) has monitored star-forming regions, and
has just begun to produce results.  To draw statistically significant
conclusions will require a much larger survey, just like CMB-S4 will provide.


==> Science/legacy_catalogs/other_maps.tex <==




==> Science/legacy_catalogs/solar_system.tex <==


\subsection{Solar System}

\label{sec:solar_system}
CMB-S4 will survey about 70\% of the sky approximately every two days. Moving objects,
such as asteroids, dwarf planets, or as yet undiscovered planets such as Planet Nine,
can be detected in difference images using their long-wavelength thermal emission. 
The expected mm-wave solar system can be seen in Fig.~\ref{fig:s4_solar_system}. For
mm-wave imaging of particular objects, an instrument like ALMA would be far more
sensitive; the particular benefit of CMB-S4 will be nearly daily measurements of
large numbers of bright objects over several years, along with wide sky coverage for
discovery of new or unexpected objects. 

Using thermal emission rather than reflected light, mm-wave measurements are less
sensitive to albedo effects, and the wavelengths are long enough that molecular
absorption and emission is negligible. Furthermore, the fall-off in flux as a function
of distance is less severe, with the main effect being the usual 1/$d^2$
dependence; optical
reflected light gets an additional factor of 1/$d^2$ from the distance to the Sun.
The temperature of solar system objects in equilibrium
with solar irradiance scales only as $d^{-1/2}$, while objects with substantial internal
heat or radioactive heating would be even less severe. 

Asteroids show substantial time variability due to rotation and viewing-angle effects.
Using CMB-S4, more than 1000 known asteroids will be detected, with many of these having
high enough signal-to-noise ratio to chart the flux as a function of rotational phase. 
Comparisons with measurements in the optical band, and also the infrared (since many of these
objects have been measured as part of the NEOWise project \cite{Masiero2018}), will yield new 
insights into the surface properties and geometry of these objects
(e.g., \cite{Mueller2017}). 

Dwarf planets, such as Pluto, will be easily detected, with measurements possible out
to roughly 100\,AU. Extending further, CMB-S4 will be able to detect any possible
planets of Earth radius or larger at about 1000\,AU. The recent excitement about
a possible Planet Nine \cite{Batygin2016}
(nominally 5--15\,$M_\oplus$ at several hundred AU) 
has made it clear that there is substantial discovery space
for new planets in the outer solar system. Assuming an earth-like composition, 
1\,$M_\oplus$ of rocky material should have an equilbrium temperature of ${>}\,30\,$K just from
radiogenic heat. An atmosphere would further enhance the mm-wave flux.
The mm-wave-sky monitoring performed by CMB-S4 offers the potential to
search for a wide variety of moving objects.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\textwidth]{Science/legacy_catalogs/s4_solar_system.png}
\caption{Millimeter-wave solar system.  Red circles show predicted asteroid flux densities at
150\,GHz, crosses show estimated flux densities of known dwarf planets at 90, 150, and 220\,GHz, and
diagonal lines show the flux density of any possible Earth-sized planet in the outer
solar system in the CMB-S4 bands. Planet 9 is estimated to be several earth masses at
a distance of several hundred AU.}
\label{fig:s4_solar_system}
\end{center}
\end{figure}



==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

